Lagrangian Motion Magnification with Double Sparse Optical Flow Decomposition

Microexpressions are fast and spatially small facial expressions that are difficult to detect. Therefore motion magnification techniques, which aim at amplifying and hence revealing subtle motion in videos, appear useful for handling such expressions. There are basically two main approaches, namely via Eulerian or Lagrangian techniques. While the first one magnifies motion implicitly by operating directly on image pixels, the Lagrangian approach uses optical flow (OF) techniques to extract and magnify pixel trajectories. In this paper, we propose a novel approach for local Lagrangian motion magnification of facial micro-motions. Our contribution is three-fold: first, we fine tune the recurrent all-pairs field transforms (RAFT) for OFs deep learning approach for faces by adding ground truth obtained from the variational dense inverse search (DIS) for OF algorithm applied to the CASME II video set of facial micro expressions. This enables us to produce OFs of facial videos in an efficient and sufficiently accurate way. Second, since facial micro-motions are both local in space and time, we propose to approximate the OF field by sparse components both in space and time leading to a double sparse decomposition. Third, we use this decomposition to magnify micro-motions in specific areas of the face, where we introduce a new forward warping strategy using a triangular splitting of the image grid and barycentric interpolation of the RGB vectors at the corners of the transformed triangles. We demonstrate the feasibility of our approach by various examples.

==> Sections/TransportEquationAnalysis.tex <==

Let us assume the simple case of a one-dimensional signal $u(x, t)$ which evolves in time \cosmas{To properly define the Forier transform later, we might also assume $u$ to live on a torus}. We can think of this signal analogously to the intensity function of our video, just in 1D. Now we assume that this signal is shifted through space with a velocity $v(t)$. We then know that under suitable regularity conditions $u$ satisfies the transport equation
$$\partial_t u = -v(t) \partial_x u.$$
In the context of motion magnification, we might want to construct a new signal $\tilde{u}$, which looks similar to $u$ in the spacial extent, but has its motion amplified by a factor of $1+\alpha$ and therefore satisfies
$$\partial_t \tilde{u} = -(1+\alpha) v(t) \partial_x \tilde{u}.$$
\\
The authors in \cite{Wu12Eulerian} approach this the following way: Construct $\tilde{u}$ by scaling certain temporal frequency bands in $u$. Writing this as a filter we get $\tilde{u} = u + u \ast b$ for a filter $b$, which extract these bands and scales them by $\alpha$. Now let us consider, how far "off" this new $\tilde{u}$ is from fulfilling the scaled transport equation:
\begin{align*}
    &\partial_t \tilde{u} + (1+\alpha) v(t) \partial_x \tilde{u}\\
    &= \partial_t u + \partial_t (u\ast b) + v(t) \partial_x u + \alpha v(t) \partial_x u + (1+\alpha)v(t) \partial_x (u \ast b)\\
    &= \partial_t u \ast b + \alpha v(t) \partial_x u + (1+\alpha)v(t) \partial_x (u \ast b)\\
    &= -(v(t) \partial_x u) \ast b + \alpha v(t) \partial_x u + (1+\alpha)v(t) \partial_x (u \ast b).
\end{align*}
Now we can ask ourselves under which conditions the L2-norm of this residual gets small. By the Plancherel theorem, we can first take a look at this expression in the frequency domain. By the convolution theorem we get
\begin{align*}
    &||\alpha \, \widehat{v} \ast \widehat{\partial_x u} + (1+\alpha) \widehat{v} \ast (\widehat{u}\, \widehat{b}) - (\widehat{v} \ast \widehat{\partial_x u})\, \widehat{b}||_2\\
    =&||(1+\alpha) \widehat{v} \ast (\widehat{u}\, \widehat{b}) - (\widehat{v} \ast \widehat{\partial_x u})\, (\widehat{b} - \alpha)||_2.
\end{align*}
$$.$$
\begin{enumerate}
    \item
    If we assume the \textbf{motion to be small in comparison with the spatial gradient of u}, we get that $u(x, \cdot)$ is nearly constant for every fixed $x$. Therefore its spectrum is concentrated around zero. Therefore, if we use a \textbf{high-pass filter $b$, which is supported away from zero}, the term $(1+\alpha) \widehat{v} \ast (\widehat{u}\, \widehat{b})$ becomes reasonably small.
    \item
    If we furthermore assume the \textbf{spectrum of $v$ to be supported away from zero}, which means that $v$ describes a non-decaying motion, we can see that $\widehat{v} \ast \widehat{\partial_x u}$ has its mass shifted away from zero. (If $v$ contains only a single frequency, this convolution shifts the majority of mass of $\widehat{\partial_x u}$, which is near zero to exactly this frequency). If we then have \textbf{the frequency response of $b$ to be near $\alpha$ in the range of frequencies of $v$}, the term $(\widehat{v} \ast \widehat{\partial_x u})\, (\widehat{b} - \alpha)$ will be small.
    \item
    As the temporal spectrum of $u$ is concentrated around zero, but nevertheless must have some mass near the frequency response of $v$ but at the same time we have to have the frequency response of $b$ to be close to $\alpha$ in this region, the magnitude of $(1+\alpha) \widehat{v} \ast (\widehat{u}\, \widehat{b})$ always eventually grows with high enough $\alpha$, so \textbf{there is no filter $b$ for which we can increase the motion magnification arbitrarily}.
\end{enumerate}
%\cosmas{As $v$ is a real function, even if its spectrum is concentrated at exactly one frequency, there will be a second peak on the negative side in the frequency domain. Therefore, in 2., the mass actually gets distributed to two peaks, which doesn't make a difference as these will be exactly mirrored as we are dealing with real signals.}

\textbf{Remark 1:}\\
For this approach to work, we must have non-uniform motion. Otherwise, we can see that for an intensity signal $u$, which satisfies the transport equation $\partial_t u = -v \partial_x u$ with constant transport velocity $v$ as well as a filter $b$ of any kind, the following holds:
$$\partial_t (u \ast b) = \partial_t u \ast b = - v \partial_x u \ast b = -v \partial_x (u \ast b),$$
i.e. in the "magnified" video, the motion remains at the same velocity $v$, just the underlying signal, which is transported, is filtered.\\

\textbf{Remark 2:}\\
In this context, the approaches from \cite{Wu12Eulerian} and \cite{DBLP:journals/corr/ZhangPG17} only differ in the frequency response of $b$ and are otherwise exactly similar.\\
\\
\textbf{Remark 3:}\\
When dividing the spatial frequencies of the image, the authors in \cite{Wu12Eulerian} show that this method is only able to magnify motions which are small compared to the spatial wavelength. They therefore suggest using different magnification factors $\alpha$ for different spatial frequencies. We can therefore analogously of our filter $b$ to be also applied in the spatial direction and having a dropoff for larger spatial frequencies. This, in turn, produces a smaller spatial second moment of the frequency response of our images which equates to less localized features on the image, i.e. $b$ is a blurring filter in the spatial extent and due to the limitations of this method, the end result will have to be blurred to some extent for larger motions.\\

==> images/sparsePCAimages/sparsePCA_tikz_figure.tex <==
\begin{tikzpicture}[scale=0.9, every node/.style={scale=0.9}]
\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0., -0.2) {\includegraphics[scale=0.2]{images/sparsePCAimages/input_smeared.png}};

\node[draw=red, line width=2pt, inner sep=0pt](n1) at (-0.57, -2.8) {\includegraphics[angle=-90, scale=0.539]{images/sparsePCAimages/normal_red.png}};

\node[draw=blue, line width=2pt, inner sep=0pt](n1) at (3.45, -0.2) {\includegraphics[scale=0.539]{images/sparsePCAimages/normal_green.png}};



\node[draw=red, line width=2pt, inner sep=0pt](n1) at (8.43, -2.8) {\includegraphics[angle = -90, scale=0.539]{images/sparsePCAimages/magnified_red.png}};

\node[draw=blue, line width=2pt, inner sep=0pt](n1) at (12.45, -0.2) {\includegraphics[scale=0.539]{images/sparsePCAimages/magnified_green.png}};


\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.4, 4.3) {\includegraphics[scale=0.2]{images/sparsePCAimages/img4.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.3, 4.2) {\includegraphics[scale=0.2]{images/sparsePCAimages/img3.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.2, 4.1) {\includegraphics[scale=0.2]{images/sparsePCAimages/img2.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.1, 4.0) {\includegraphics[scale=0.2]{images/sparsePCAimages/img1.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0, 3.9) {\includegraphics[scale=0.2]{images/sparsePCAimages/img0.png}};



\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.4, 10.4) {\includegraphics[scale=0.2]{images/sparsePCAimages/flow4.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.3, 10.3) {\includegraphics[scale=0.2]{images/sparsePCAimages/flow3.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.2, 10.2) {\includegraphics[scale=0.2]{images/sparsePCAimages/flow2.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.1, 10.1) {\includegraphics[scale=0.2]{images/sparsePCAimages/flow1.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (0.0, 10.0) {\includegraphics[scale=0.2]{images/sparsePCAimages/flow0.png}};


\node[](n1) at (10, 11) {\includegraphics[scale=0.35]{images/sparsePCAimages/code_graphs.png}};


\node[](n1) at (7.5, 7.35) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component0.png}};
\node[](n1) at (10, 7.35) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component2.png}};
\node[](n1) at (12.5, 7.35) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component3.png}};
\node[](n1) at (7.5, 5.45) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component1.png}};
\node[](n1) at (10, 5.45) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component5.png}};
\node[](n1) at (12.5, 5.45) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component6.png}};
\node[](n1) at (7.5, 3.55) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component7.png}};
\node[](n1) at (10, 3.55) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component8.png}};
\node[](n1) at (12.5, 3.55) {\includegraphics[width=2.4cm]{images/sparsePCAimages/component9.png}};

\node[draw=black, line width=2pt, inner sep=0pt](n1) at (9, -0.2) {\includegraphics[scale=0.2]{images/sparsePCAimages/output_smeared.png}};


%\node[](n2) at (0.2, 2.1) {Input frames};

\draw[-{Triangle[width=18pt,length=8pt]}, line width=10pt](-1,6.4) -- (-1, 8.1);

\draw[-{Triangle[width=18pt,length=8pt]}, line width=10pt](3,9.5) -- (5, 9.5);

\draw[-{Triangle[width=18pt,length=8pt]}, line width=10pt](8,2.5) -- (8, 1.7);

\node[](n2) at (1.1, 7.4) {Optical flow estimation};
\node[](n2) at (4, 8.9) {Sparse PCA};
\node[](n2) at (10.7, 2.1) {Adaptive motion magnification};

\end{tikzpicture}
